TSUE: A Two-Stage Data Update Method for an Erasure Coded Cluster File System

Compared to replication-based storage systems, erasure-coded storage incurs significantly higher overhead during data updates. To address this issue, various parity logging methods have been pro- posed. Nevertheless, due to the long update path and substantial amount of random I/O involved in erasure code update processes, the resulting long latency and low throughput often fail to meet the requirements of high performance applications. To this end, we propose a two-stage data update method called TSUE. TSUE divides the update process into a synchronous stage that records updates in a data log, and an asynchronous stage that recycles the log in real-time. TSUE effectively reduces update latency by transforming random I/O into sequential I/O, and it significantly reduces recycle overhead by utilizing a three-layer log and the spatio-temporal locality of access patterns. In SSDs cluster, TSUE significantly im- proves update performance, achieving improvements of 7.6X under Ali-Cloud trace, 5X under Ten-Cloud trace, while it also extends the SSD's lifespan by up to 13X through reducing the frequencies of reads/writes and of erase operations.

==> List-Update/Tab-2-test.tex <==
\begin{tabular}{|c|ccc|ccc|ccc|c|}
\hline
\multirow{2}{*}{\textbf{TRACE}} & \multicolumn{3}{c|}{\textbf{DATA\_LOG}} & \multicolumn{3}{c|}{\textbf{DELTA\_LOG}} & \multicolumn{3}{c|}{\textbf{PARITY\_LOG}}     & \multirow{2}{*}{\textbf{\begin{tabular}[c|]{@{}c@{}}TOTAL\\ TIME\end{tabular}}}   \\ \cline{2-10} 

& \multicolumn{1}{c|}{APPE.$^{\mathrm{1}}$} & \multicolumn{1}{c|}{BUFF.$^{\mathrm{2}}$}  & \multicolumn{1}{c|}{RECY.$^{\mathrm{3}}$} &
\multicolumn{1}{c|}{APPE.$^{\mathrm{1}}$} & \multicolumn{1}{c|}{BUFF.$^{\mathrm{2}}$}  & \multicolumn{1}{c|}{RECY.$^{\mathrm{3}}$} &
\multicolumn{1}{c|}{APPE.$^{\mathrm{1}}$} & \multicolumn{1}{c|}{BUFF.$^{\mathrm{2}}$}  & \multicolumn{1}{c|}{RECY.$^{\mathrm{3}}$} & \\ \hline
                                
\textbf{Ali-Cloud}              & \multicolumn{1}{c|}{107}    & \multicolumn{1}{c|}{1561410} & \multicolumn{1}{c|}{350}  & \multicolumn{1}{c|}{75}    & \multicolumn{1}{c|}{6846260} & \multicolumn{1}{c|}{526} & \multicolumn{1}{c|}{136}    & \multicolumn{1}{c|}{742066} & \multicolumn{1}{c|}{434}  & \multicolumn{1}{c|}{9151364}   \\ \hline

\textbf{Ten-Cloud}              & \multicolumn{1}{c|}{96}   & \multicolumn{1}{c|}{4388070} & \multicolumn{1}{c|}{323} & \multicolumn{1}{c|}{185}    & \multicolumn{1}{c|}{59434880} & \multicolumn{1}{c|}{237}   & \multicolumn{1}{c|}{218}    & \multicolumn{1}{c|}{64447} & \multicolumn{1}{c|}{2363} &  \multicolumn{1}{c|}{10979659}  \\ \hline

\multicolumn{11}{l}{NOTE: APP.$^{\mathrm{1}}$ is the item insert into log; BUFF.$^{\mathrm{2}}$ is the residence time of a log entry in the log; RECY.$^{\mathrm{3}}$ is the item in log is recycled} \\
\multicolumn{11}{l}{The Execution is performed under RS(12,4).} \\
\end{tabular}


==> List-Update/Tab-3.tex <==
% \begin{tabular}{|c|cc|cc|c|}
% \hline
% \multirow{2}{*}{\textbf{METHOD}} & \multicolumn{2}{c|}{\textbf{READ/WRITE in SSD}}                              & \multicolumn{2}{c}{\textbf{OVERWRITE(Write Penalty)}}   &   \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}NETWORK\\ TRAFFIC\end{tabular}}}                      \\ \cline{2-5} 
%                         &   \multicolumn{1}{c|}{\textbf{Num.} }     & \textbf{Volume(GB)} & \multicolumn{1}{c|}{\textbf{Num.}} & \textbf{Volume(GB)}\\ \hline


% \textbf{FO}              & \multicolumn{1}{c|}{9739320}    & \multicolumn{1}{c|}{894} & \multicolumn{1}{c|}{4869660}   & \multicolumn{1}{c|}{447}     & 447     \\ \hline


% \textbf{PL}              & \multicolumn{1}{c|}{13726649}   & \multicolumn{1}{c|}{1252} & \multicolumn{1}{c|}{4869660}   & \multicolumn{1}{c|}{447}    & 447    \\ \hline

% \textbf{PLR}              & \multicolumn{1}{c|}{8860540}   & \multicolumn{1}{c|}{1240} & \multicolumn{1}{c|}{7493637}   & \multicolumn{1}{c|}{440}     & 447  \\ \hline

% \textbf{PARIX}              & \multicolumn{1}{c|}{6439527}   & \multicolumn{1}{c|}{471} & \multicolumn{1}{c|}{1456968}   & \multicolumn{1}{c|}{96}     & 454   \\ \hline

% \textbf{TSUE}              & \multicolumn{1}{c|}{1776864}   & \multicolumn{1}{c|}{555} & \multicolumn{1}{c|}{401466}   & \multicolumn{1}{c|}{223}    & 383    \\ \hline
% \multicolumn{6}{l}{Running in RS(6,4) with Ten-Cloud.} \\
% \end{tabular}

\begin{tabular}{|cccccc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{METHOD}}} & \multicolumn{2}{c|}{\textbf{READ/WRITE}}                               & \multicolumn{2}{c|}{\textbf{OVERWRITE(Write Penalty)}}                        & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}NETWORK\\ TRAFFIC(GB)\end{tabular}}} \\ \cline{2-5}
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{\textbf{Num.}} & \multicolumn{1}{c|}{\textbf{Volume(GB)}} & \multicolumn{1}{c|}{\textbf{Num.}} & \multicolumn{1}{c|}{\textbf{Volume(GB)}} &                                                                                     \\ \hline
\multicolumn{1}{|c|}{\textbf{FO}}                      & \multicolumn{1}{c|}{9739320}       & \multicolumn{1}{c|}{894}                 & \multicolumn{1}{c|}{4869660}       & \multicolumn{1}{c|}{447}                 & 447                                                                                 \\ \hline
\multicolumn{1}{|c|}{\textbf{PL}}                      & \multicolumn{1}{c|}{13726649}      & \multicolumn{1}{c|}{1252}                & \multicolumn{1}{c|}{4869660}       & \multicolumn{1}{c|}{447}                 & 447                                                                                 \\ \hline
\multicolumn{1}{|c|}{\textbf{PLR}}                     & \multicolumn{1}{c|}{8860540}       & \multicolumn{1}{c|}{1240}                & \multicolumn{1}{c|}{7493637}       & \multicolumn{1}{c|}{440}                 & 447                                                                                 \\ \hline
\multicolumn{1}{|c|}{\textbf{PARIX}}                   & \multicolumn{1}{c|}{6439527}       & \multicolumn{1}{c|}{471}                 & \multicolumn{1}{c|}{1456968}       & \multicolumn{1}{c|}{96}                  & 454       \\ \hline

\multicolumn{1}{|c|}{\textbf{CoRD}}                    & \multicolumn{1}{c|}{2913936}       & \multicolumn{1}{c|}{365}                 & \multicolumn{1}{c|}{1094691}        & \multicolumn{1}{c|}{271}                 & 276    \\ \hline 

\multicolumn{1}{|c|}{\textbf{TSUE}}                    & \multicolumn{1}{c|}{\textbf{2750796}}       & \multicolumn{1}{c|}{645}                 & \multicolumn{1}{c|}{\textbf{401466}}        & \multicolumn{1}{c|}{\textbf{223}}                 & 290    \\ \hline                                                            

\multicolumn{6}{l}{Replaying Ten-Cloud Trace in RS(6,4).}   
\footnote{To ensure reliability, the data logs and delta logs in TSUE use the dual-copy mechanism, and all the logs in TSUE are persisted to SSDS. When a node crashes, the lost log data can be read from the replica log in other nodes, and the parity log data can be obtained through the recovery process.}

\end{tabular}

\begin{comment}
    \multicolumn{1}{|c|}{\textbf{TSUE}}                    & \multicolumn{1}{c|}{\textbf{1776864}}       & \multicolumn{1}{c|}{555}                 & \multicolumn{1}{c|}{\textbf{401466}}        & \multicolumn{1}{c|}{223}                 & 383/290    \\ \hline
\end{comment}
